Ladder Symmetries of Black Holes: Implications for Love Numbers and No-Hair Theorems

It is well known that asymptotically flat black holes in general relativity have a vanishing static, conservative tidal response. We show that this is a result of linearly realized symmetries governing static (spin 0,1,2) perturbations around black holes. The symmetries have a geometric origin: in the scalar case, they arise from the (E)AdS isometries of a dimensionally reduced black hole spacetime. Underlying the symmetries is a ladder structure which can be used to construct the full tower of solutions, and derive their general properties: (1) solutions that decay with radius spontaneously break the symmetries, and must diverge at the horizon; (2) solutions regular at the horizon respect the symmetries, and take the form of a finite polynomial that grows with radius. Taken together, these two properties imply that static response coefficients -- and in particular Love numbers -- vanish. Moreover, property (1) is consistent with the absence of black holes with linear (perturbative) hair. We also discuss the manifestation of these symmetries in the effective point particle description of a black hole, showing explicitly that for scalar probes the worldline couplings associated with a non-trivial tidal response and scalar hair must vanish in order for the symmetries to be preserved.

==> pgflibraryvectorian.code.tex <==
% pgflibraryvectorian.code.tex (utf8 encoding)
% Copyright 2020  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status “maintained”.
% 
% The Current Maintainer of this work is Alain Matthes.
% Original idea of  F Fradin and H Voss  
\typeout{2020/04/06 1.1  pgflibraryvectorian.code.tex} 
\makeatletter
% dimensions des motifs
\def\@pgfornamentDim#1{% dim en bp
\ifcase#1\relax%
\or\def\@pgfornamentX{136}\def\@pgfornamentY{107}% 1
\or\def\@pgfornamentX{134}\def\@pgfornamentY{48}%  2
\or\def\@pgfornamentX{130}\def\@pgfornamentY{65}%  3
\or\def\@pgfornamentX{133}\def\@pgfornamentY{133}% 4
\or\def\@pgfornamentX{129}\def\@pgfornamentY{146}% 5
\or\def\@pgfornamentX{134}\def\@pgfornamentY{148}% 6
\or\def\@pgfornamentX{136}\def\@pgfornamentY{135}% 7
\or\def\@pgfornamentX{134}\def\@pgfornamentY{134}% 8
\or\def\@pgfornamentX{79}\def\@pgfornamentY{105}% 9
\or\def\@pgfornamentX{80}\def\@pgfornamentY{99}%  10
\or\def\@pgfornamentX{123}\def\@pgfornamentY{67}%  11
\or\def\@pgfornamentX{136}\def\@pgfornamentY{136}% 12
\or\def\@pgfornamentX{136}\def\@pgfornamentY{236}% 13
\or\def\@pgfornamentX{123}\def\@pgfornamentY{67}%  14
\or\def\@pgfornamentX{103}\def\@pgfornamentY{52}%  15
\or\def\@pgfornamentX{103}\def\@pgfornamentY{52}%  16
\or\def\@pgfornamentX{74}\def\@pgfornamentY{59}%  17
\or\def\@pgfornamentX{74}\def\@pgfornamentY{59}%  18
\or\def\@pgfornamentX{81}\def\@pgfornamentY{81}%  19
\or\def\@pgfornamentX{81}\def\@pgfornamentY{81}%  20
\or\def\@pgfornamentX{70}\def\@pgfornamentY{58}%  21
\or\def\@pgfornamentX{34}\def\@pgfornamentY{61}%  22
\or\def\@pgfornamentX{68}\def\@pgfornamentY{55}%  23
\or\def\@pgfornamentX{79}\def\@pgfornamentY{76}%  24
\or\def\@pgfornamentX{80}\def\@pgfornamentY{88}%  25
\or\def\@pgfornamentX{59}\def\@pgfornamentY{120}% 26
\or\def\@pgfornamentX{101}\def\@pgfornamentY{98}% 27
\or\def\@pgfornamentX{52}\def\@pgfornamentY{102}% 28
\or\def\@pgfornamentX{65}\def\@pgfornamentY{65}%  29
\or\def\@pgfornamentX{63}\def\@pgfornamentY{64}%  30
\or\def\@pgfornamentX{48}\def\@pgfornamentY{48}%  31
\or\def\@pgfornamentX{48}\def\@pgfornamentY{48}%  32
\or\def\@pgfornamentX{85}\def\@pgfornamentY{85}%  33
\or\def\@pgfornamentX{85}\def\@pgfornamentY{85}%  34
\or\def\@pgfornamentX{97}\def\@pgfornamentY{97}%  35
\or\def\@pgfornamentX{97}\def\@pgfornamentY{97}%  36
\or\def\@pgfornamentX{105}\def\@pgfornamentY{104}% 37
\or\def\@pgfornamentX{105}\def\@pgfornamentY{104}% 38
\or\def\@pgfornamentX{112}\def\@pgfornamentY{112}% 39
\or\def\@pgfornamentX{112}\def\@pgfornamentY{112}% 40
\or\def\@pgfornamentX{111}\def\@pgfornamentY{113}% 41
\or\def\@pgfornamentX{111}\def\@pgfornamentY{113}% 42
\or\def\@pgfornamentX{123}\def\@pgfornamentY{63}%  43
\or\def\@pgfornamentX{123}\def\@pgfornamentY{63}%  44
\or\def\@pgfornamentX{385}\def\@pgfornamentY{64}%  45
\or\def\@pgfornamentX{453}\def\@pgfornamentY{97}%  46
\or\def\@pgfornamentX{114}\def\@pgfornamentY{32}%  47
\or\def\@pgfornamentX{114}\def\@pgfornamentY{32}%  48
\or\def\@pgfornamentX{163}\def\@pgfornamentY{61}%  49
\or\def\@pgfornamentX{164}\def\@pgfornamentY{125}% 50
\or\def\@pgfornamentX{164}\def\@pgfornamentY{125}% 51
\or\def\@pgfornamentX{248}\def\@pgfornamentY{197}% 52
\or\def\@pgfornamentX{134}\def\@pgfornamentY{134}% 53
\or\def\@pgfornamentX{134}\def\@pgfornamentY{134}% 54
\or\def\@pgfornamentX{269}\def\@pgfornamentY{116}% 55
\or\def\@pgfornamentX{269}\def\@pgfornamentY{116}% 56
\or\def\@pgfornamentX{207}\def\@pgfornamentY{103}% 57
\or\def\@pgfornamentX{228}\def\@pgfornamentY{116}% 58
\or\def\@pgfornamentX{204}\def\@pgfornamentY{102}% 59
\or\def\@pgfornamentX{451}\def\@pgfornamentY{189}% 60
\or\def\@pgfornamentX{205}\def\@pgfornamentY{205}% 61
\or\def\@pgfornamentX{205}\def\@pgfornamentY{205}% 62
\or\def\@pgfornamentX{212}\def\@pgfornamentY{212}% 63
\or\def\@pgfornamentX{212}\def\@pgfornamentY{212}% 64
\or\def\@pgfornamentX{132}\def\@pgfornamentY{166}% 65
\or\def\@pgfornamentX{177}\def\@pgfornamentY{175}% 66
\or\def\@pgfornamentX{80}\def\@pgfornamentY{155}% 67
\or\def\@pgfornamentX{361}\def\@pgfornamentY{154}% 68
\or\def\@pgfornamentX{448}\def\@pgfornamentY{227}% 69
\or\def\@pgfornamentX{226}\def\@pgfornamentY{79}%  70
\or\def\@pgfornamentX{443}\def\@pgfornamentY{81}%  71
\or\def\@pgfornamentX{216}\def\@pgfornamentY{58}%  72
\or\def\@pgfornamentX{216}\def\@pgfornamentY{58}%  73
\or\def\@pgfornamentX{308}\def\@pgfornamentY{93}%  74
\or\def\@pgfornamentX{373}\def\@pgfornamentY{120}% 75
\or\def\@pgfornamentX{308}\def\@pgfornamentY{93}%  76
\or\def\@pgfornamentX{207}\def\@pgfornamentY{89}%  77
\or\def\@pgfornamentX{207}\def\@pgfornamentY{132}% 78
\or\def\@pgfornamentX{249}\def\@pgfornamentY{122}% 79
\or\def\@pgfornamentX{454}\def\@pgfornamentY{31}%  80
\or\def\@pgfornamentX{176}\def\@pgfornamentY{45}%  81
\or\def\@pgfornamentX{454}\def\@pgfornamentY{24}%  82
\or\def\@pgfornamentX{449}\def\@pgfornamentY{20}%  83
\or\def\@pgfornamentX{290}\def\@pgfornamentY{57}%  84
\or\def\@pgfornamentX{453}\def\@pgfornamentY{22}%  85
\or\def\@pgfornamentX{454}\def\@pgfornamentY{17}%  86
\or\def\@pgfornamentX{360}\def\@pgfornamentY{44}%  87
\or\def\@pgfornamentX{454}\def\@pgfornamentY{15}%  88
\or\def\@pgfornamentX{454}\def\@pgfornamentY{10}%  89
\or\def\@pgfornamentX{30}\def\@pgfornamentY{30}%  90
\or\def\@pgfornamentX{44}\def\@pgfornamentY{29}%   91
\or\def\@pgfornamentX{43}\def\@pgfornamentY{29}%   92
\or\def\@pgfornamentX{59}\def\@pgfornamentY{29}%   93
\or\def\@pgfornamentX{59}\def\@pgfornamentY{29}%   94
\or\def\@pgfornamentX{43}\def\@pgfornamentY{29}%   95
\or\def\@pgfornamentX{30}\def\@pgfornamentY{15}%   96
\or\def\@pgfornamentX{29}\def\@pgfornamentY{14}%   97
\or\def\@pgfornamentX{29}\def\@pgfornamentY{14}%   98
\or\def\@pgfornamentX{45}\def\@pgfornamentY{15}%   99
\or\def\@pgfornamentX{29}\def\@pgfornamentY{30}%   100
\or\def\@pgfornamentX{132}\def\@pgfornamentY{30}%  101
\or\def\@pgfornamentX{43}\def\@pgfornamentY{29}%102
\or\def\@pgfornamentX{42}\def\@pgfornamentY{30}%103
\or\def\@pgfornamentX{44}\def\@pgfornamentY{29}%104
\or\def\@pgfornamentX{45}\def\@pgfornamentY{30}%105
\or\def\@pgfornamentX{44}\def\@pgfornamentY{30}%106
\or\def\@pgfornamentX{44}\def\@pgfornamentY{29}%107
\or\def\@pgfornamentX{59}\def\@pgfornamentY{29}%108
\or\def\@pgfornamentX{72}\def\@pgfornamentY{29}%109
\or\def\@pgfornamentX{29}\def\@pgfornamentY{15}%110
\or\def\@pgfornamentX{43}\def\@pgfornamentY{28}%111
\or\def\@pgfornamentX{15}\def\@pgfornamentY{59}%112
\or\def\@pgfornamentX{57}\def\@pgfornamentY{28}%113
\or\def\@pgfornamentX{44}\def\@pgfornamentY{29}%114
\or\def\@pgfornamentX{43}\def\@pgfornamentY{29}%115
\or\def\@pgfornamentX{29}\def\@pgfornamentY{29}%116
\or\def\@pgfornamentX{29}\def\@pgfornamentY{29}%117
\or\def\@pgfornamentX{29}\def\@pgfornamentY{29}%118
\or\def\@pgfornamentX{44}\def\@pgfornamentY{29}%119
\or\def\@pgfornamentX{29}\def\@pgfornamentY{44}%120
\or\def\@pgfornamentX{30}\def\@pgfornamentY{44}%121
\or\def\@pgfornamentX{44}\def\@pgfornamentY{29}%122
\or\def\@pgfornamentX{59}\def\@pgfornamentY{29}%123
\or\def\@pgfornamentX{58}\def\@pgfornamentY{59}%124
\or\def\@pgfornamentX{30}\def\@pgfornamentY{44}%125
\or\def\@pgfornamentX{29}\def\@pgfornamentY{43}%126
\or\def\@pgfornamentX{44}\def\@pgfornamentY{28}%127
\or\def\@pgfornamentX{45}\def\@pgfornamentY{29}%128
\or\def\@pgfornamentX{44}\def\@pgfornamentY{29}%129
\or\def\@pgfornamentX{29}\def\@pgfornamentY{29}%130
\or\def\@pgfornamentX{45}\def\@pgfornamentY{44}%131
\or\def\@pgfornamentX{45}\def\@pgfornamentY{44}%132
\or\def\@pgfornamentX{15}\def\@pgfornamentY{15}%133
\or\def\@pgfornamentX{15}\def\@pgfornamentY{15}%134
\or\def\@pgfornamentX{15}\def\@pgfornamentY{14}%135
\or\def\@pgfornamentX{72}\def\@pgfornamentY{44}%136
\or\def\@pgfornamentX{149}\def\@pgfornamentY{74}%137
\or\def\@pgfornamentX{15}\def\@pgfornamentY{7}%138
\or\def\@pgfornamentX{73}\def\@pgfornamentY{37}%139
\or\def\@pgfornamentX{15}\def\@pgfornamentY{15}%140
\or\def\@pgfornamentX{15}\def\@pgfornamentY{15}%141
\or\def\@pgfornamentX{30}\def\@pgfornamentY{30}%142
\or\def\@pgfornamentX{30}\def\@pgfornamentY{30}%143
\or\def\@pgfornamentX{29}\def\@pgfornamentY{30}%144
\or\def\@pgfornamentX{15}\def\@pgfornamentY{15}%145
\or\def\@pgfornamentX{15}\def\@pgfornamentY{15}%146
\or\def\@pgfornamentX{31}\def\@pgfornamentY{29}%147
\or\def\@pgfornamentX{30}\def\@pgfornamentY{44}%148
\or\def\@pgfornamentX{29}\def\@pgfornamentY{28}%149
\or\def\@pgfornamentX{30}\def\@pgfornamentY{44}%150
\or\def\@pgfornamentX{43}\def\@pgfornamentY{29}%151
\or\def\@pgfornamentX{57}\def\@pgfornamentY{28}%152
\or\def\@pgfornamentX{57}\def\@pgfornamentY{28}%153
\or\def\@pgfornamentX{34}\def\@pgfornamentY{17}%154
\or\def\@pgfornamentX{34}\def\@pgfornamentY{17}%155
\or\def\@pgfornamentX{45}\def\@pgfornamentY{28}%156
\or\def\@pgfornamentX{44}\def\@pgfornamentY{29}%157
\or\def\@pgfornamentX{58}\def\@pgfornamentY{29}%158
\or\def\@pgfornamentX{43}\def\@pgfornamentY{29}%159
\or\def\@pgfornamentX{43}\def\@pgfornamentY{30}%160
\or\def\@pgfornamentX{44}\def\@pgfornamentY{29}%161
\or\def\@pgfornamentX{30}\def\@pgfornamentY{44}%162
\or\def\@pgfornamentX{46}\def\@pgfornamentY{29}%163
\or\def\@pgfornamentX{29}\def\@pgfornamentY{44}%164
\or\def\@pgfornamentX{45}\def\@pgfornamentY{26}%165
\or\def\@pgfornamentX{44}\def\@pgfornamentY{29}%166
\or\def\@pgfornamentX{44}\def\@pgfornamentY{29}%167
\or\def\@pgfornamentX{59}\def\@pgfornamentY{30}%168
\or\def\@pgfornamentX{58}\def\@pgfornamentY{29}%169
\or\def\@pgfornamentX{59}\def\@pgfornamentY{30}%170
\or\def\@pgfornamentX{30}\def\@pgfornamentY{29}%171
\or\def\@pgfornamentX{29}\def\@pgfornamentY{15}%172
\or\def\@pgfornamentX{29}\def\@pgfornamentY{44}%173
\or\def\@pgfornamentX{28}\def\@pgfornamentY{44}%174
\or\def\@pgfornamentX{29}\def\@pgfornamentY{42}%175
\or\def\@pgfornamentX{29}\def\@pgfornamentY{43}%176
\or\def\@pgfornamentX{31}\def\@pgfornamentY{44}%177
\or\def\@pgfornamentX{28}\def\@pgfornamentY{44}%178
\or\def\@pgfornamentX{29}\def\@pgfornamentY{44}%179
\or\def\@pgfornamentX{30}\def\@pgfornamentY{45}%180
\or\def\@pgfornamentX{43}\def\@pgfornamentY{30}%181
\or\def\@pgfornamentX{45}\def\@pgfornamentY{29}%182
\or\def\@pgfornamentX{44}\def\@pgfornamentY{27}%183
\or\def\@pgfornamentX{42}\def\@pgfornamentY{29}%184
\or\def\@pgfornamentX{45}\def\@pgfornamentY{29}%185
\or\def\@pgfornamentX{43}\def\@pgfornamentY{14}%186
\or\def\@pgfornamentX{28}\def\@pgfornamentY{29}%187
\or\def\@pgfornamentX{30}\def\@pgfornamentY{30}%188
\or\def\@pgfornamentX{44}\def\@pgfornamentY{29}%189
\or\def\@pgfornamentX{44}\def\@pgfornamentY{29}%190
\or\def\@pgfornamentX{73}\def\@pgfornamentY{58}%191
\or\def\@pgfornamentX{29}\def\@pgfornamentY{44}%192
\or\def\@pgfornamentX{44}\def\@pgfornamentY{14}%193
\or\def\@pgfornamentX{90}\def\@pgfornamentY{90}%194
\or\def\@pgfornamentX{90}\def\@pgfornamentY{90}%195
\or\def\@pgfornamentX{148}\def\@pgfornamentY{30}%196

\fi%
}%
\makeatother
\endinput
